A Descending Price Auction for Matching Markets

This work presents a descending-price-auction algorithm to obtain the maximum market-clearing price vector (MCP) in unit-demand matching markets with m items by exploiting the combinatorial structure. With a shrewd choice of goods for which the prices are reduced in each step, the algorithm only uses the combinatorial structure, which avoids solving LPs and enjoys a strongly polynomial runtime of $O(m^4)$. Critical to the algorithm is determining the set of under-demanded goods for which we reduce the prices simultaneously in each step of the algorithm. This we accomplish by choosing the subset of goods that maximize a skewness function, which makes the bipartite graph series converges to the combinatorial structure at the maximum MCP in $O(m^2)$ steps. A graph coloring algorithm is proposed to find the set of goods with the maximal skewness value that yields $O(m^4)$ complexity.

==> Sections/VI_Discussion.tex <==
%!TEX root = ../main.tex

\section{Discussions}   \label{sec6}

    %\subsection{Same bipartite graph in each rounds does not imply the same set of MCPs}

    We now discuss some interesting points of the choices made in our algorithm, some nuances in terms of the final bipartite graphs, and a few comments on the non-monotonicity of bidding with strategic concerns.

    \subsection{Choice of Constricted Goods Set} \label{sec6.1}

		Suppose we do not choose the most skewed set in our algorithm, then it follows that we may obtain different MCP vectors. However, a natural question to ask is the following: if we run the algorithm two times and choose different constricted good sets at some iterations such that the bipartite graph produced in every round of these two executions are the same, will we get the same MCP vector?
		
        Unfortunately, the choice of the same initial price vector, the same price reduction rule, and the emergence of the same bipartite graph in every round are not enough to guarantee the same returned MCPs. A counterexample is provided in Fig. \ref{fig4}.
	
	\begin{figure}[h]
	\centering
        \includegraphics[width=0.4\textwidth]{./Figures/constricted.pdf}
        \caption{Counterexample of same bipartite graph but different set MCPs}
        \label{fig4}
    \end{figure}

    In Fig. \ref{fig4}, the bipartite graphs A-1, B-1 have the same preference graph. Though the chosen constricted good sets in A, B are different, they add the same buyer to the constricted graph. Therefore, the preference graphs in A-2, B-2 are still the same. However, the updated price vector of A-2, B-2 must be different. If A, B choose the same constricted goods set in every round, the returned sets of MCPs of A, B must be different. This example shows that just the bipartite graphs in every round cannot uniquely determine the MCP vector obtained at the termination of the algorithm.

	\subsection{Failure of Connectivity in Matching Markets} \label{sec6.3}
    In general matching markets, the set of goods in the bipartite graph is not always connected, even at the maximum MCP. A disconnected structure in bipartite graph implies a set of buyers' bids/values may play no role on another set of buyers' payment in the MCP. In other words, a set of buyers will be indifferent when another sets of buyers bids/values are within specific regions;  this phenomenon happens when sets of buyers have greater affinity for some pre-determined types of goods, i.e., valuation of men and women on ties and high heels would satisfy such a property. In sponsored search markets, however, the set of goods in the initial bipartite graph is connected\footnote{Every good is preferred by the buyer with the highest bid.}. Furthermore, the following lemma shows that our skewed-set aided descending price algorithm will preserve the connectivity property in all iterations, and therefore also at termination.
     	\begin{lem} \label{lem8}
			In sponsored search markets with the skewed-set aided descending price algorithm, any set of goods in every bipartite graph that is encountered during the execution of Algorithm \ref{alg:alg1} is connected.
		\end{lem}
		\begin{proof}
           Please see Appendix~\ref{sec:lem8}.
	    \end{proof}
In Lemma~\ref{lem8}, we addressed the connectivity property in sponsored search markets during the execution of our algorithm. Unfortunately, the connectivity does not always hold in general matching markets. Here we demonstrate this by a $4$-by-$4$ counter example below.
	
		To make this case as simple as possible, we just consider a realized valuation matrix 	
		\begin{eqnarray*}
		V=
		\begin{bmatrix}
    	5 & 4 & 1 & 1 \\
    	3 & 3 & 2 & 2 \\
    	2 & 2 & 3 & 3 \\
    	1 & 1 & 4 & 5
		\end{bmatrix}.			
		\end{eqnarray*}
		
		Initially, the first two goods are preferred by buyer 1, and the last two goods are preferred by buyer buyer 4. In our algorithm, the most skewed set contains all goods, and price is reduced by one in the first round. After that, the MCP vector $\mathbf{P}=[4,3,3,4]$ and the bipartite graphs of initial and final steps are in Fig. \ref{fig:connectivity}.
	\begin{figure}[h]
	\centering
       \includegraphics[width=0.4\textwidth]{./Figures/connectivity.pdf}
        \caption{An example where both initial and final bipartite graphs are disconnected}
        \label{fig:connectivity}
    \end{figure}
		
	Fig. \ref{fig:connectivity} demonstrates that both the initial and final bipartite graphs are disconnected in our algorithm as there are two components. Therefore, preserving the connectivity property in the running of our algorithm holds in sponsored search markets, and may not otherwise.

    \subsection{Further Comments on Strategic Bidding}

    Unlike most of the non-incentive compatible auction mechanisms that overbidding above buyers' actual value is always irrational, a buyer may benefit from bidding higher than her actual value to enjoy a lower price under the proposed algorithm in some scenarios. We can show this by a simple example below.
    
    First, we present two valuations matrices that will yield the same matching but different prices with the difference in the matrices only being the valuations of one buyer. These are
    		\begin{eqnarray*}
		V_1=
		\begin{bmatrix}
    	4 & 5 & 5 & 6 \\
    	2 & 4 & 5 & 5 \\
    	1 & 2 & 4 & 5 \\
    	0 & 1 & 2 & 4
		\end{bmatrix}, \quad
        		V_2 =
		\begin{bmatrix}
    	4 & 5.9 & 5.9 & 6.9 \\
    	2 & 4 & 5 & 5 \\
    	1 & 2 & 4 & 5 \\
    	0 & 1 & 2 & 4
		\end{bmatrix}.
		\end{eqnarray*}
        The maximum MCPs  are $P_1=[1, 2, 3, 4]$ and $P_2=[0.1,2,3,4]$, respectively, and in both cases buyer $i$ gets matched to good $i$ for all $i\in \{1,\dotsc,4\}$. Now if we assume that the true valuations of all the buyers is given by matrix $V_1$, then by unilaterally deviating to a higher bid, buyer $1$ is able to dramatically increase her payoff without impacting any other buyers. While this is only an example, we believe that this will occur with non-zero probability and will necessitate an alternate means of determining the equilibrium bidding behavior.
	

==> Sections/V_Analysis_G.tex <==
%!TEX root = ../main.tex

\section{Preliminary Analysis of Strategic Buyers and Bayesian-Nash Equilibrium} \label{sec5}

As mentioned in the introduction, the proposed descending price algorithm is not incentive compatible, and so we need to explore Bayesian Nash equilibrium (BNE) to predict buyers' strategic behaviors. From the messaging viewpoint we will assume that we have a direct mechanism where the buyers bid their valuation: a scalar in sponsored search markets, and a vector in the general matching market. Algorithm \ref{alg:alg1} is then applied as a black-box to the inputs to produce a price on each good and a perfect matching. With expected revenue being an important concern, we provide an instance achieving higher expected revenue than VCG mechanism in an asymmetric BNE. Furthermore, a case provided to show the possibility of overbidding. Additional analyses of BNE in two simple cases with symmetric buyers and the associated bidding strategy of the buyers are provided in Appendices \ref{apdx:analysis} and \ref{apdx:analysis2}.

\subsection{An Instance Achieving higher expected revenue than VCG}\label{sec:greatRev}

	Given the proposed algorithm, it is important to check if there exists a scenario that our algorithm obtain a higher expected revenue than the VCG mechanism. There is a large body of literature discussing the failure of getting the VCG revenue under asymmetric distribution of buyers' valuations, e.g., see \cite{VCGfailure}. Additionally, the well-known revenue equivalence theorem holds with an assumption that valuation of every player is drawn from a path-connected space in Chap. 9.6.3 of \cite{SSMbook}\footnote{Two other assumptions are (1) both mechanisms implement the same social welfare function; (2) for every player $i$, there exists a type that the expected payments are the same in both mechanisms}. With this knowledge, we demonstrate a $3\times 3$ matching market, where the buyers have asymmetric distributions of their valuations, for which our mechanism achieves higher than VCG revenue. 

    Consider three advertisers named Alice, Bob, and Carol, and three different types of ads called listing ads, sidebar ads, and pop-ups. The realized valuation is only known to the advertiser (equivalently buyer), but the distribution of an advertisers' valuation is known to other advertisers but not the auctioneer. In other words, the auctioneer can only calculate the price according to the bids submitted by the advertisers. The minimum increment of the submitted bids is $\epsilon$, which is a positive infinitesimal, and the valuation matrix of advertisers is displayed in Table \ref{tbl:1}.
    %\gs{There appears to be a typo in the table!  First $f_y(y)$ should not have a 2 in it.  Second, why is the notation so odd $f_y(y)$ lists $y$ twice, $y$?}
    \begin{table}[h]
\centering
\caption{Valuation matrix of advertisers}
\label{tbl:1}
\begin{tabular}{|l|l|l|l|} \hline
      & Listing & Sidebar & Pop-ups   \\ \hline
Alice & W & 0 & 0   \\ \hline
Bob   & X & 0  & 0.5 \\ \hline
Carol & Y & Z & 2    \\ \hline
\end{tabular} \\
\begin{tabular}{|ll|} \hline
Probability density function of $W,X,Y,Z$ &\\ \hline
$f_W(w)=\begin{cases}
	\frac{2}{3} &~w\in [0,1) \\
    \frac{1}{3} &~w\in (2,3] \\
    0 &~\text{o/w}
	 \end{cases} $ &
$f_X(x)=\begin{cases}
	\frac{2}{3} &~x\in [1.5,2.5] \\
    \frac{1}{3} &~x\in (2.5,3.5] \\
    0 &~\text{o/w}
	 \end{cases}$      \\
$f_Y(y)=\begin{cases}
	2 &~y\in [3.5,4] \\
    0 &~\text{o/w}
	 \end{cases}$
&$f_Z(z)=\begin{cases}
	1 &~z\in [3,4] \\
    0 &~\text{o/w}
	 \end{cases}   $  \\ \hline
\end{tabular}
\end{table}

Now, we give an asymmetric BNE\footnote{Multiple equilibria may exist.} in this matching market, with a detailed verification in the Appendix \ref{asymBNE}. First, assume that Alice always bids 0 on sidebar ads and pop-ups, and bids $\max \{1-\epsilon, \frac{w}{2}\}$ on listing ads. The best response of Bob is to bid 0 on both sidebar ads and pop-ups, and to bid $\max \{1, \frac{x-0.5}{2}\}$ on listing ads for any realized $x$. Now, given Bob's bidding function as above, one of Alice's best responses is to follow her original bidding function. Last, consider the bidding function of Alice and Bob mentioned above, a best response of Carol is to bid 0 on listing ads and pop-ups, and to bid $\epsilon$ on sidebar ads regardless of the outcomes of $y$ and $z$.   %\gs{changed this, I hope its clearer/correct} %for every positive realized $y,z$
\footnote{The $\epsilon$ is designed to avoid complex tie-breaking rules.}, even if $y>z$. This is because Carol will never win listing ads for any bids less than $1$ as the probability $\text{Pr}\{y-z \geq 1\}=0$. Now, given Carol's bidding strategy, Alice and Bob will not change their bidding functions. Therefore, the strategy $\{\beta_{\mathrm{Alice}}(w,0,0), \beta_{\mathrm{Bob}}(x,0,0.5),\beta_{\mathrm{Carol}}(y,z,2)\}=\{(\max \{1-\epsilon, \frac{w}{2}\},0,0), (\max \{1, \frac{2x-1}{4}\},0,0),(0,\epsilon,0)\}$ can be verified to be an asymmetric BNE.

	With the asymmetric BNE in hand, we want to calculate the expected revenue of the auctioneer and compare it with the expected revenue of the VCG mechanism. Since Carol always wins the sidebar ads and both Alice and Bob bid 0 on that, Carol will pay $\epsilon$. Additionally, in the asymmetric BNE, Alice and Bob compete on the listing ads and both bid 0 on sidebar ads and pop-ups, resulting in the payment of listing ads to be the same as the payment in the first price auction. Using this the expected revenue of the auctioneers is given by
    \begin{eqnarray}
    &&\epsilon+\frac{4}{9}\int_0^1\int_{1.5}^{2.5} 1 dxdw+\frac{2}{9}\int_2^3\int_{1.5}^{2.5} \frac{w}{2} dxdw+\frac{2}{9}\int_1^2\int_{2.5}^{3.5} \frac{2x-1}{4} dxdw \nonumber \\&+&\frac{1}{9}\int_2^3\int_{2.5}^{w+0.5} \frac{w}{2} dxdw+\frac{1}{9}\int_{2.5}^{3.5}\int_2^{x-0.5} \frac{2x-1}{4} dwdx =\dfrac{31}{27}+\epsilon
    \end{eqnarray}
The last step is to calculate the expected revenue of the VCG mechanism, which is given by
    \begin{eqnarray}
    &&\frac{2}{3}\int_0^1\int_{1.5}^{2.5} w dxdw+\frac{2}{9}\int_2^3\int_{1.5}^{2.5} (x-0.5) dxdw+\frac{1}{9}\int_{2.5}^{3.5}\int_2^{x-0.5} w dwdx \nonumber \\&+&\frac{1}{9}\int_2^3\int_{2.5}^{w+0.5} (x-0.5) dxdw =\dfrac{1}{3}+\dfrac{2}{9}\times \dfrac{3}{2}+\dfrac{1}{9}\times \dfrac{7}{6}++\dfrac{1}{9}\times \dfrac{7}{6}=\dfrac{25}{27}
    \end{eqnarray}
Even if we set $\epsilon$ to 0, it is obvious that the expected revenue derived under our descending price auction algorithm is strictly greater than the expected revenue of the VCG mechanism. This shows that in some instances the proposed descending price algorithm is preferred to the (DGS) ascending price algorithm,  even taking the strategic behavior of buyers into account.

    \subsection{Further Comments on Strategic Bidding}

    Unlike most of the non-incentive compatible auction mechanisms where overbidding above buyers' actual value is always irrational, in some scenarios a buyer may benefit from bidding higher than her actual value to enjoy a lower price in the proposed algorithm. We show this by a simple example below.
    
    First, we present two valuations matrices that will yield the same matching but different prices with the difference in the matrices only being the valuations of one buyer. These are
    		\begin{eqnarray*}
		V_1=
		\begin{bmatrix}
    	4 & 5 & 5 & 6 \\
    	2 & 4 & 5 & 5 \\
    	1 & 2 & 4 & 5 \\
    	0 & 1 & 2 & 4
		\end{bmatrix}, \quad
        		V_2 =
		\begin{bmatrix}
    	4 & 5.9 & 5.9 & 6.9 \\
    	2 & 4 & 5 & 5 \\
    	1 & 2 & 4 & 5 \\
    	0 & 1 & 2 & 4
		\end{bmatrix}.
		\end{eqnarray*}
        The maximum MCPs  are $P_1=[1, 2, 3, 4]$ and $P_2=[0.1,2,3,4]$, respectively, and in both cases buyer $i$ gets matched to good $i$ for all $i\in \{1,\dotsc,4\}$. Now if we assume that the true valuations of all the buyers is given by matrix $V_1$, then by unilaterally deviating to a higher bid on three goods, buyer $1$ is able to dramatically increase her payoff without impacting any other buyer. While this is only an example, we believe that this will occur with non-zero probability and will necessitate an alternate means of determining the equilibrium bidding behavior.
